M2H2: A Multimodal Multiparty Hindi Dataset For Humor Recognition in Conversations

Humor recognition in conversations is a challenging task that has recently gained popularity due to its importance in dialogue understanding, including in multimodal settings (i.e., text, acoustics, and visual). The few existing datasets for humor are mostly in English. However, due to the tremendous growth in multilingual content, there is a great demand to build models and systems that support multilingual information access. To this end, we propose a dataset for Multimodal Multiparty Hindi Humor (M2H2) recognition in conversations containing 6,191 utterances from 13 episodes of a very popular TV series "Shrimaan Shrimati Phir Se". Each utterance is annotated with humor/non-humor labels and encompasses acoustic, visual, and textual modalities. We propose several strong multimodal baselines and show the importance of contextual and multimodal information for humor recognition in conversations. The empirical results on M2H2 dataset demonstrate that multimodal information complements unimodal information for humor recognition. The dataset and the baselines are available at http://www.iitp.ac.in/~ai-nlp-ml/resources.html and https://github.com/declare-lab/M2H2-dataset.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typset multiple affiliations (Christoph Sommer)

==> ch3-related-work.tex <==
% \section{Related Work}\label{related-work}

% % In this section, we describe 

% \subsection{Unimodal Humor}
% Humor is one of the affective states of human behaviour that is not very easy to understand and interpret. %Humor is a global and basic feelings that everyone understands. 
% %Text is humorous or not is now very common task. 
% Some of the prior research have focused on understanding humors %Lots of research
% \cite{bolkan2018humor,scheel2017definitions,boykoff2019laughing,gal2019ironic,weller2019humor,blinov2019large}. % has been already done to understand the behaviour of humor. 
% \cite{weller2019humor} proposed a transformer based architecture to detect that joke is funny or not. The author collected the jokes on the basis of rating gleaned from Reddit pages which contains 16000 labelled instances.  

% Castro et al. \cite{castro2017crowd} presented a collection of 27,000 tweets published in Spanish that have been crowd-sourced for their comedy value and funniness score. Weber et al. \cite{weber2018shape} developed a reinforcement learning-based dynamic user modeling technique. Lexical features are very much important in humor detection. Zhao et al. \cite{zhao2019embedding} proposed a novel tensor embedding method that can effectively extract lexical features for humor recognition. The author used word-to-word co-occurrence to encode the contextual content of documents. For filling in the blanks in Mad Libs® tales, \cite{garimella2020judge} present an automated humor generating system. They extended the BERT platform to predict location-biased word fills in incomplete sentences and fine-tuned BERT to categorize sentence-level location-specific comedy.  

% % Humor/Laughter may be used by health care practitioners and educators to promote health and teaching and learning. Savage et al. \cite{savage2017humor} discussed brief review on Humor, laughter, learning, and health. Fry et al. \cite{fry1994biology} summarized key themes concerning the interactions between humor and biology. Whereas, Veatch et al. \cite{veatch1998theory} examined that humor is an apparent condition of emotional absurdity in which the observed situation appears to be normal.






% % \cite{wellenzohn2018benefits} wanted to see if personality qualities and sense of humor may help to mitigate the long-term effects of humor-based therapies on happiness and depressive symptoms. So, the author conducted two studies and claimed that humor-based therapies were found to be equally effective for both humorous and non-humorous persons, however improvements in sense of humor throughout the intervention phase may serve as an indicator of whether the intervention should be continued in the long run. Warren et al. \cite{warren2018humor} created a framework for comprehending the various methods in which laughing and humor assist customers in achieving their objectives. 

% The Humor Styles Questionnaire (HSQ) distinguishes four types of humor that can be good or damaging to one's mental health. \cite{schneider2018joke} studied to compile research that used the HSQ to analyze the relationships between distinct humor types and four distinct aspects of mental health (self-esteem, life satisfaction, optimism, depression). While, Fritz et al. \cite{fritz2017humor} examined three studies and found that humor that was dispositional, self-enhancing, affiliative, or self-defeating had a direct effect on distress that was mediated by social contact and reappraisal.
% % \textcolor{red}{ Stress-relieving benefits were seen in both dispositional and aggressive humor. }

% % According to race researchers, the modern era of "race relations" is characterized by a "color-blind" racial ideology. Racist humor is identified as a language that opposes such limits on public racist discourse in \cite{perez2017racism}. Racist humor helps interlocutors to build social interactions by participating in the "forbidden fruit" in a post-civil-rights and color-blind society.


% % Bolkan et al. \cite{bolkan2018humor} investigated the effects of integrated humor on pupils' capacity to retain and transfer information. They did two experiments, to know the relation to the potential for humor and distraction in the classroom. According to the findings, Those exposed to the hilarious condition did lower on their examinations than students exposed to the regular cases. In other work, Scheel et al. \cite{scheel2017definitions} presented an overview of humor conceptualizations, the most popular ideas, and ideas that might be used as a framework for work-related comedy research. Humor is a multifaceted concept that encompasses the talents to create, identify, and appreciate humor. 




% % While, Gal et al. \cite{gal2019ironic} examined the use of irony in social media for boundary work. They explored the manner in which online irony acts as a social consolidation and distinction by using the example of left-wing ridicule of a far-right-wing group in Israel.

% % Humor and comedy are increasingly being used to communicate about climate change in a culturally relevant way. According to critics, humor serves as a diversion from the seriousness of climate change issues. \cite{boykoff2019laughing} investigated the potential for humor and humor to influence new ways of thinking and acting regarding anthropogenic climate change. It studies how sensory, emotional, and aesthetic learning might inform scientific ways of knowing in a critical way.

% \subsection{Code-mixed Humor}
% While posting on social media, users frequently switch between languages, a practice known as code-mixing. It raises certain issues in the realm of social media content analysis. To identify comedy, a deep semantic comprehension of the text is necessary, making the task challenging to automate. Khandelwal et al. \cite{khandelwal2018humor} described a publicly accessible corpus of English-Hindi code-mixed tweets tagged with humorous(H) or non-humorous(N) tags in this study. In another work, Sane et al. \cite{sane2019deep} presented multilingual word embeddings based on word2vec and fastText models. They attempted to solve the difficulty of detecting humor in Hindi-English code-mixed tweets. They offered models that use the created bilingual embeddings as input, such as convolutional neural networks (CNN) and bidirectional long-short term memory (biLSTM) (with and without Attention). 








% \subsection{Multimodal Humor}
% As we have already discussed that sometimes just going through the utterance text is not enough to understand humor. Sometimes visual and acoustic both are important for some tasks while sometimes all the three modalities i.e., text, acoustic, and visual are important. In natural language processing, understanding humor from these modalities comes under the boundaries of multimodal language. Humor may be found in almost every human-to-human encounter. Some works \cite{hasan2019ur,fallianda2018analyzing,ritschel2019irony,ritschel2020multimodal,mirnig2017elements,piata2020stylistic,song2021humor,vasquez2021cats,sabur2020identification,veronika2020multimodal,yang2019multimodal} on multimodal humor have already been done.

% Hasan et al. \cite{hasan2019ur} proposed the UR-FUNNY dataset to aid in the comprehension of multimodal language utilized in the expression of humor. The author has also shown the importance of multimodality over uni-modality. Humor can be created with any of modalities. Fallianda et al. \cite{fallianda2018analyzing} looked at how humor was created using only verbal media, both verbal and visual media, and exclusively visual media. The data was gathered from 74 political comic strips published in Kompas newspaper. The author used the General Theory of Verbal Humor (GTVH) for humor analysis.

% Higher pitch or loudness, a faster speaking cadence, or considerable pauses are not characteristics of conversational humor. In the paper, \cite{attardo2011prosodic} discovered that when people are laughing or smiling, they are more likely to be humorous. El and Nabiha \cite{el2020multimodal} did two experiments: the first experiment looks at whether untrained people can recognize the structural aspects of humor in a multimodal text. The second research investigates the sequence in which textual and visual inputs are processed (tweets). In another work, Ritschel et al. \cite{ritschel2019irony} find that the quality of a conversation and how conversation partners see one other can be influenced by irony and irony-related humor. 

% % Prochazka et al. \cite{prochazka2016cohesive} investigated the ability of online memes to bring people together in the communal and multimodal environment of Facebook. The report suggests that the community's cohesion is based on its proclivity towards linguistic and social uniformity. 'Classical Art Memes' are humorous internet memes based on classical and medieval art. According to the \cite{piata2020stylistic} findings, memes communicate emotional meanings that derive from the embodied emotion in the textually recontextualized picture. Adding to the body of knowledge about online memes and humor, Vasquez et al. \cite{vasquez2021cats} looked at a series of picture macros associated with a particular viral media incident. In this work they gathered 220 image macros linked to this media event from three different Internet sources. Multiple instances of wordplay utilizing paronymy and register-based comedy are shown in the findings.

% % The human is usually the one who writes the robot's jokes. Ritschel et al. \cite{ritschel2020multimodal} showcased a socially aware robot that creates multimodal jokes. It adapts a paralinguistic presenting method based on socially conscious reinforcement learning, which reads human social cues and attempts to increase user humor. Sabur et al. \cite{sabur2020identification} figured out the multimodal structure of humor in an animated superhero film. The qualitative descriptive approach was utilized, with the goal of discovering potential humor. The findings reveal that the cartoon film has two types of humor. 

% % Humor is created in cartoons through two semiotic modes: verbal and visual, or just via the visual form. Tsakona et al. \cite{tsakona2009language} used a General Theory of Verbal Humor (GTVH) framework with cognitive and semiotic techniques to show that humor in cartoons is not always easy to grasp fully and the reader should capture each single detail of each cartoon. The goal of the research was to take the GTVH one step closer to unifying linguistic and semiotic approaches to comedy. Sabur et al. \cite{sabur2020identification} figured out the multimodal structure of humor in an animated superhero film. The qualitative descriptive approach was utilized, with the goal of discovering potential humor. The findings reveal that the cartoon film has two types of humor.

% % Veronika et al. \cite{veronika2020multimodal} looked at how picture books use humor to stimulate dialogue and fulfill its interpersonal role. The Systemic Functional Approach to Multimodal Discourse Analysis was used to analyze multimodal hilarious events (SF-MDA). In the context of traditional incongruity theory of humor, Chen et al. \cite{chen2018you} examined humor via the prism of prototype theory. It aspires to a linguistic and semiotic approach to humor that is cohesive. Yang et al. \cite{yang2019multimodal} proposed a machine learning technique for generating unsupervised humor labels in films using time-aligned user comments. In other work, Song et al. \cite{song2021humor} looked at how students in an online multimodal learning environment developed and shared humor. On a social-networking website, 28 students contributed 1006 pins that were submitted to a multimodal content analysis. Some pins that were not meant to be humorous ended up being used as instances of comedy.

% In comparison to the existing systems, we first created the \textit{Multimodal Multi-party Hindi Humorous Dataset} (M2H2) by manually labeling each utterance with humor/non-humor and addressee information. Thereafter, we employ two strong baselines for humor recognition. Further, to the best of our knowledge, this is the very first attempt at solving the humor detection in Hindi conversational setting. Empirical results on the \textit{M2H2} dataset demonstrate that the baselines yields better performance over the single-task framework.











==> tex/comparativeResults.tex <==
\begin{table*}[!h]
\centering
\resizebox{1\textwidth}{!}
{    
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c||c|c|c|c|c|c|c|c|c|}

\hline
& \multicolumn{9}{c||}{\bf \em Speaker Dependent} & \multicolumn{9}{c|}{\bf \em Speaker Independent} \\ \hline

& \multicolumn{3}{c|}{\bf Proposed} & \multicolumn{3}{c|}{\bf Baseline-1 \shortcite{castro2019towards}} & \multicolumn{3}{c||}{\bf Baseline-2 \shortcite{chauhan-etal-2020-sentiment}}  & \multicolumn{3}{c|}{\bf Proposed} &  \multicolumn{3}{c||}{\bf Baseline-1 \shortcite{castro2019towards}} &  \multicolumn{3}{c|}{\bf Baseline-2 \shortcite{chauhan-etal-2020-sentiment} }  \\
\cline{2-19}
\multicolumn{1}{|c|}{\bf \em Labels} & \bf P & \bf R & \bf F1 & \bf P & \bf R & \bf F1 & \bf P & \bf R & \bf F1  & \bf P & \bf R & \bf F1 & \bf P & \bf R & \bf F1 & \bf P & \bf R & \bf F1  \\ \hline \hline
% \multirow{2}{*}{\em\begin{tabular}{@{}c@{}}Speaker\\Dependent\end{tabular}} & \multirow{1}{*}{ \em STL} & \bf \em Sar & 71.52 & 70.61 & 69.32 & 64.20 & 64.20 & 63.88 & 71.90 & 71.01 & 70.64  \\
% \cline{2-12}
\bf \em T & \bf 69.9 & \bf 69.7 & \bf 69.6 & 65.1 & 64.6 & 64.6 & - & - & - & \bf 63.1 & \bf 61.2 & \bf 62.0 & 60.9 & 59.6 & 59.8 & - & - & -  \\
\bf \em A & \bf 69.1 & \bf 68.0 & \bf 67.4 & 65.9 & 64.6 & 64.6 & - & - & - & \bf 67.2 & \bf 67.4 & \bf 67.3 & 65.1 & 62.6 & 62.7 & - & - & -  \\
\bf \em V & \bf 75.1 & \bf 74.2 & \bf 74.0 & 68.1 & 67.4 & 67.4 & - & - & - & \bf 65.4 & \bf 65.7 & \bf 65.5 & 54.9 & 53.4 & 53.6 & - & - & -  \\ \hline
\bf \em T+V & \bf 75.1 & \bf 74.8 & \bf 74.7 & 72.0 & 71.6 & 71.6 & 72.7 &  71.9 & 71.6 & \bf 66.2 & \bf 66.6 & \bf 66.2 & 62.2 & 61.5 & 61.7 & 65.5 & 65.5 & 65.7  \\
\bf \em T+A & \bf 70.6 & \bf 70.3 & \bf 70.1 & 66.6 & 66.2 & 66.2 & 62.2 & 61.1 & 59.6 & \bf 69.5 & \bf 66.0 & \bf 65.9 & 64.7 & 62.9 & 63.1 & 59.1 & 60.0 & 50.3  \\
\bf \em A+V & \bf 76.1 & \bf 75.7 & \bf 75.6 & 66.2 & 65.7 & 65.7 & 72.7 & 71.9 & 71.8 & \bf 68.9 & \bf 69.1 & \bf 68.2 & 64.1 & 61.8 & 61.9 & 65.6 & 63.8 & 63.9  \\ \hline
\bf \em T+V+A & \bf 77.9 & \bf 76.9 & \bf 76.7 & 71.9 & 71.4 & 71.5 & 73.4 & 72.7 & 72.6 & \bf 70.1 & \bf 69.7 & \bf 69.8 & 64.3 & 62.6 & 62.8 & 69.5 & 66.0 & 65.9  \\


\hline
\end{tabular}
}
\caption{Comparative analysis between our proposed model, and Baseline-1 and Baseline-2 for the \textit{w/o context and w/o speaker} setups }
\label{tab:comparative_analysis}
\end{table*}















% \begin{table*}[!h]
% \centering
% \resizebox{0.95\textwidth}{!}
% {    
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c||c|c|c|}

% \hline
% \multirow{2}{*}{\bf \em Setup}& \multirow{2}{*}{\bf \em Model} & \multicolumn{3}{c|}{\bf T +  V } &  \multicolumn{3}{c|}{\bf T + A } &  \multicolumn{3}{c||}{\bf A + V} &  \multicolumn{3}{|c|}{\bf T + A + V}\\ \cline{3-14}
% & & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 \\
% \hline
% \hline
% \multirow{3}{*}{\em\begin{tabular}{@{}c@{}}Speaker\\Dependent\end{tabular}} & \bf \em Baseline & 72.0 & 71.6 & 71.6 & \bf 66.6 & \bf 66.2 & \bf 66.2 & 66.2 & 65.7 & 65.7 & 71.9 & 71.4 & 71.5 \\
% % \cline{2-14}
% & \bf \em Proposed Model & \bf 72.8 & \bf 71.9 & \bf 71.6 & 62.2 & 61.2 & 59.6 & \bf 72.7 & \bf 71.9 & \bf 71.8 & \bf 73.4 & \bf 72.8 & \bf 72.6 \\
% \cline{2-14}
% & \textit{T}-test & - & - & - & - & - & - & - & - & - & 0.0023 & 0.0098 & 0.0056\\ 
% \hline
% \hline
% \multirow{3}{*}{\em\begin{tabular}{@{}c@{}}Speaker\\ Independent\end{tabular}} & \bf \em Baseline & 62.2 & 61.5 & 61.7 & \bf 64.7 & \bf 62.9 & \bf 63.1 & 64.1 & 61.8 & 61.9 & 64.3 & 62.6 & 62.8 \\
% % \cline{2-14}
% & \bf \em Proposed Model & \bf 65.5 & \bf 65.5 & \bf 65.7 & 59.1 & 60.0 & 50.3 & \bf 65.6 & \bf 63.8 & \bf 63.9 & \bf 69.5 & \bf 66.0 & \bf 65.9 \\
% \cline{2-14}
% & \textit{T}-test & - & - & - & - & - & - & - & - & - & 0.0002 & 0.0006  & 0.0012 \\
% \hline
% \end{tabular}
% }
% % \caption{Comparative Analysis}
% \caption{Comparative Analysis of the proposed approach with recent state-of-the-art systems. We evaluated on extended, publicly available MUSTARD dataset \cite{castro2019towards}. Significance test \textit{p}-values$<0.05$}
% \label{tab:comparative_analysis}
% \end{table*}

% %================================================================================================

% % \begin{table*}[!h]
% % \centering
% % \resizebox{0.95\textwidth}{!}
% % {    
% % \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c||c|c|c|}

% % \hline
% % \multirow{2}{*}{\bf \em Setup}& \multirow{2}{*}{\bf \em Model} & \multicolumn{3}{c|}{\bf T +  V } &  \multicolumn{3}{c|}{\bf T + A } &  \multicolumn{3}{c||}{\bf A + V} &  \multicolumn{3}{|c|}{\bf T + A + V}\\ \cline{3-14}
% % & & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 \\
% % \hline
% % \hline
% % \multirow{2}{*}{\em\begin{tabular}{@{}c@{}}Speaker\\Dependent\end{tabular}} & \bf \em Baseline & 72.0 & 71.6 & 71.6 & \bf 66.6 & \bf 66.2 & \bf 66.2 & 66.2 & 65.7 & 65.7 & 71.9 & 71.4 & 71.5 \\
% % % \cline{2-14}
% % & \bf \em Proposed Model & \bf 72.76 & \bf 71.88 & \bf 71.61 & 62.23 & 61.15 & 59.61 & \bf 72.73 & \bf 71.88 & \bf 71.81 & \bf 73.40 & \bf 72.75 & \bf 72.57 \\
% % \hline
% % \hline
% % \multirow{2}{*}{\em\begin{tabular}{@{}c@{}}Speaker\\ Independent\end{tabular}} & \bf \em Baseline & 62.2 & 61.5 & 61.7 & \bf 64.7 & \bf 62.9 & \bf 63.1 & 64.1 & 61.8 & 61.9 & 64.3 & 62.6 & 62.8 \\
% % % \cline{2-14}
% % & \bf \em Proposed Model & \bf 65.48 & \bf 65.48 & \bf 65.67 & 59.13 & 59.98 & 50.27 & \bf 65.59 & \bf 63.76 & \bf 63.90 & \bf 69.53 & \bf 66.01 & \bf 65.90 \\
% % \hline
% % \end{tabular}
% % }
% % \caption{Comparative Analysis}
% % \label{tab:comparative_analysis}
% % \end{table*}


% % =========================================================================


% % \begin{table*}[!h]
% % \centering
% % \resizebox{0.9\textwidth}{!}
% % {    
% % \begin{tabular}{|c|c|c|c|c|c|c||c|c|c|c|c|c|c|c|c| }

% % \hline
% % \multicolumn{16}{|c|}{\bf \em Speaker Dependent} \\ \hline
% % & \multicolumn{3}{c|}{\bf \em Baseline } & \multicolumn{3}{c|}{\bf \em Sar + Sent + Emo} &  \multicolumn{3}{c|}{\bf \em Sar + Sent} &  \multicolumn{3}{c|}{\bf \em Sar + Emo} &  \multicolumn{3}{c|}{\bf \em Sar}\\
% % \cline{2-16}
% % \bf \em Labels & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 \\ 
% % \hline
% % \hline
% % \bf  T + V     &  72.0 & 71.6 & 71.6 & \bf 72.76 & \bf 71.88 & \bf 71.61 & 69.65 & 69.42 & 69.33 & 71.76 & 70.86 & 70.54 & 71.52 & 70.61 & 69.32 \\
% % \bf  T + A     &  \bf 66.6 & \bf 66.2 & \bf 66.2 & 63.23 & 61.15 & 59.61 & 64.09 & 60.72 & 58.21 &  65.76 &  65.65 &  65.60 & 64.20 & 64.20 & 63.88\\
% % \bf  A + V     &  66.2 & 65.7 & 65.7  & \bf 72.73 & \bf 71.88 & \bf 71.81 & 72.20 & 71.45 & 71.18 & 72.60 & 71.59 & 71.25 & 71.90 & 71.01 & 70.64\\ \hline
% % \bf  T + A + V &  71.9 & 71.4 & 71.5 & \bf 73.40 & \bf 72.75 & \bf 72.57 & 72.52 & 71.73 & 71.47 & 72.76 & 71.88 & 72.11 & 72.08 & 71.62 & 72.01\\
% % \hline
% % \end{tabular}
% % }
% % \caption{Multimodal : Speaker Dependent Setups}
% % \label{tab:speaker_dependent_multimodal}
% % \end{table*}


% % % ===========================================================
% % \begin{table*}[!h]
% % \centering
% % \resizebox{0.9\textwidth}{!}
% % {    
% % % \begin{tabular}{|c| p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|}
% % \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c| }

% % \hline
% % \multicolumn{16}{|c|}{\bf \em Speaker Independent} \\ \hline
% % &  \multicolumn{3}{c|}{\bf \em Baseline }  & \multicolumn{3}{c|}{\bf \em Sar + Sent + Emo} &  \multicolumn{3}{c|}{\bf \em Sar + Sent} &  \multicolumn{3}{c|}{\bf \em Sar + Emo} &  \multicolumn{3}{c|}{\bf \em Sar}\\
% % \cline{2-16}
% % \bf \em Labels & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1  & P & R & F1 \\ 
% % \hline
% % \hline
% % \bf  T + V     & 62.2 & 61.5 & 61.7  & \bf 65.48 & \bf 65.48 & \bf 65.67 & 62.74 & 62.92 & 62.81 & 65.11 & 65.16 & 65.13 & 60.11 & 60.18 & 60.16\\
% % \bf  T + A     & \bf  64.7 & \bf 62.9 & \bf 63.1  & 59.13 & 58.98 & 50.27 & 59.25 & 59.55 & 52.89 &  59.59 &  59.55 &  59.58 & 58.23 & 57.69 & 57.91\\
% % \bf  A + V     & 64.1 & 61.8 & 61.9 & \bf 65.59 & \bf 63.76 & \bf 63.90 & 61.60 & 60.95 & 61.14 & 63.19 & 63.76 & 62.91 & 60.44 & 60.96 & 60.52 \\ \hline  
% % \bf  T + A + V & 64.3 & 62.6 & 62.8 & \bf 69.53 & \bf 66.01 & \bf 65.90 & 66.97 & 63.76 & 63.68 & 66.35 & 65.44 & 65.63 & 65.98 & 65.45 & 65.60\\
% % \hline
% % \end{tabular}
% % }
% % \caption{Multimodal : Speaker Independent Setups}
% % \label{tab:speaker_independent_multimodal}
% % \end{table*}


==> tex/dataset_samples.tex <==
\begin{table}[!h]
\small
\centering
\resizebox{0.49\textwidth}{!}
{
% \begin{tabular}{|p{20em}|C{3.5em}|C{4.25em}|C{10em}|} \hline
\begin{tabular}{|l|p{20em}||c|}
\hline
% & & \multicolumn{2}{c||}{\bf \em Dataset samples} \\ \cline{3-7}
\bf No. & \bf Utterances & \bf Emoji  \\ \hline \hline
1 & \textit{It's just a privilege to watch your mind at work.} & \includegraphics[scale=2.21]{images/emojis/table1.pdf}   \\  \hline

2 & \textit{To feed the cat Rose.} & \includegraphics[scale=0.084]{images/emojis/table5.pdf} \\  \hline

3 & \textit{You're kidding, right?} & \includegraphics[scale=2.21]{images/emojis/table3.pdf}  \\  \hline

4 & \textit{Could you be more specific?} & \includegraphics[scale=2.21]{images/emojis/table4.pdf}  \\  \hline

5 & \textit{Oh my God I love that! - Really? - NO!} & \includegraphics[scale=2.21]{images/emojis/abstract1.pdf}  \\  \hline \hline

\multicolumn{3}{|c|}{\bf Emojis used for annotation} \\ \hline

\multicolumn{3}{|c|}{\includegraphics[scale=0.018]{images/emojis/Anger_high_anger.pdf}\includegraphics[scale=0.018]{images/emojis/Anger_low_anger.pdf}\includegraphics[scale=0.018]{images/emojis/Excited_sparkel.pdf}\includegraphics[scale=0.018]{images/emojis/Excited_huggingface.pdf}\includegraphics[scale=0.018]{images/emojis/Fear_low_fear.pdf}\includegraphics[scale=0.018]{images/emojis/Fear_high_fear.pdf}\includegraphics[scale=0.018]{images/emojis/Sad_emojiwithtear.pdf}\includegraphics[scale=0.018]{images/emojis/Sad_sad3.pdf}\includegraphics[scale=0.018]{images/emojis/Sad_sad.pdf}\includegraphics[scale=0.018]{images/emojis/Surprised_roundeyes.pdf}\includegraphics[scale=0.018]{images/emojis/Surprised_openmouth.pdf}\includegraphics[scale=0.018]{images/emojis/Frustrated_low.pdf}\includegraphics[scale=0.018]{images/emojis/Frustated_high.pdf}\includegraphics[scale=0.018]{images/emojis/Happy_rollingfacelaugh.pdf}\includegraphics[scale=0.018]{images/emojis/Happy_kissing.pdf}\includegraphics[scale=0.018]{images/emojis/Happy_smile_eyes.pdf}\includegraphics[scale=0.018]{images/emojis/Happy_lougheyeswithtear.pdf}\includegraphics[scale=0.018]{images/emojis/Happy_beatingheart.pdf}\includegraphics[scale=0.018]{images/emojis/Happy_heart_eyes.pdf}\includegraphics[scale=0.018]{images/emojis/Happy_teethshowing.pdf}\includegraphics[scale=0.018]{images/emojis/Neutral_neutral.pdf}
\includegraphics[scale=0.018]{images/emojis/Neutral_eyesneutral.pdf}\includegraphics[scale=0.018]{images/emojis/Disgust_zikzak.pdf}\includegraphics[scale=0.018]{images/emojis/Disgust_pukeface.pdf}\includegraphics[scale=0.018]{images/emojis/Disgust_potty.pdf}} \\ \hline


\end{tabular}
}
\caption{Dataset samples
}
\label{tab-dataset_table}
\end{table}

% \begin{table}[t]
% \centering
% % \arraystretch{1.3}
% \resizebox{0.35\textwidth}{!}
% {
% \begin{tabular}{l|c|c}
% \hline
% \bf Emoji & $E^m_s$  & $E^m_e$\\  \hline \hline

% % \multirow{1}{*}{ Bi-LSTM+Attn}  & 2(Layers)*128  ,Dropout=0.05 \\ 
                          
% % \multirow{1}{*}{ FC}  & 2*128, Dropout=0.05 \\ 
% % \multicolumn{1}{|c|}{\multirow{6}{*}{\bf \em \begin{turn}{90}Input\end{turn}}}
% \includegraphics[scale=0.018]{images/emojis/Anger_high_anger.pdf} \includegraphics[scale=0.018]{images/emojis/Anger_low_anger.pdf}  & Neg & Anger  \\ 

% \includegraphics[scale=0.018]{images/emojis/Excited_sparkel.pdf} \includegraphics[scale=0.018]{images/emojis/Excited_huggingface.pdf}  & Pos & Excited  \\ 


%  \includegraphics[scale=0.018]{images/emojis/Fear_low_fear.pdf} \includegraphics[scale=0.018]{images/emojis/Fear_high_fear.pdf}  & Neg & Fear  \\ 

% \includegraphics[scale=0.018]{images/emojis/Sad_emojiwithtear.pdf}
% \includegraphics[scale=0.018]{images/emojis/Sad_sad3.pdf} \includegraphics[scale=0.018]{images/emojis/Sad_sad.pdf}  & Neg & Sad  \\ 

%  \includegraphics[scale=0.018]{images/emojis/Surprised_roundeyes.pdf} \includegraphics[scale=0.018]{images/emojis/Surprised_openmouth.pdf}  & Pos & Surprised  \\ 

%  \includegraphics[scale=0.018]{images/emojis/Frustrated_low.pdf} \includegraphics[scale=0.018]{images/emojis/Frustated_high.pdf}  & Neg & Frustrated  \\ 


% \includegraphics[scale=0.018]{images/emojis/Happy_rollingfacelaugh.pdf} 
% \includegraphics[scale=0.018]{images/emojis/Happy_kissing.pdf} 
% \includegraphics[scale=0.018]{images/emojis/Happy_smile_eyes.pdf} 
% \includegraphics[scale=0.018]{images/emojis/Happy_lougheyeswithtear.pdf} 
%  \includegraphics[scale=0.018]{images/emojis/Happy_beatingheart.pdf} 
% \includegraphics[scale=0.018]{images/emojis/Happy_heart_eyes.pdf} 
% \includegraphics[scale=0.018]{images/emojis/Happy_teethshowing.pdf}  & Pos & Happy  \\ 

%  \includegraphics[scale=0.018]{images/emojis/Neutral_neutral.pdf} \includegraphics[scale=0.018]{images/emojis/Neutral_eyesneutral.pdf} & Neutral & Neutral  \\ 

% \includegraphics[scale=0.018]{images/emojis/Disgust_zikzak.pdf}
%  \includegraphics[scale=0.018]{images/emojis/Disgust_pukeface.pdf} \includegraphics[scale=0.018]{images/emojis/Disgust_potty.pdf}  & Neg & Disgust  \\ 



% \hline    

% \end{tabular}
% }
% \caption{Emoji description.}
% \label{tab:emoji_description}
% \end{table}




==> tex/error_analysis_right_prediction.tex <==
\begin{table}[!h]
\small
\centering
\resizebox{0.49\textwidth}{!}
{
% \begin{tabular}{|p{20em}|C{3.5em}|C{4.25em}|C{10em}|} \hline
\begin{tabular}{|l|p{18em}||c||c|c| }
\hline
& & & \multicolumn{2}{c|}{\bf \em Predicted} \\ \cline{4-5}

& \bf  & \bf  & \bf Unimodal & \bf Multimodal \\ 
& \bf Utterances & \bf Actual & \bf (T) & \bf (T+V+A) \\ \hline \hline

1 & \begin{hindi} अरे बुढ़ापे में मैं तुम्हें खुद ले के जाता।अरे बुढ़ापे में मैं तुम्हें खुद ले के जाता। \end{hindi}
& humor & \textcolor{red}{non-humor} & humor \\ \hline

2 & \begin{hindi} ये दिलरुबा कहता है ना कि पिछले जन्म में वो छोटूमल मोटूमल करोड़पति का एकलौता बेटा था, राइट? \end{hindi}
& non-humor & \textcolor{red}{humor} & non-humor \\ \hline

3 & \begin{hindi} स्टाफ वालों! मेरा मतलब \end{hindi} 
& humor & \textcolor{red}{non-humor} & humor \\ \hline

4 & \begin{hindi} कुछ याद आया? कुछ याद आया? \end{hindi} 
& non-humor & \textcolor{red}{humor} & non-humor \\ \hline

5 & \begin{hindi} जाते वक्त ऐसी अशुभ बातें नहीं करते। \end{hindi} 
& humor & \textcolor{red}{non-humor} & humor  \\ \hline

\end{tabular}
}
% \caption{Some incorrectly predicted samples by the proposed model.}
\caption{Some correctly predicted samples}
\label{tab-error_analysis_correct_prediction}
\end{table}


% ================================================================================
% \begin{table*}[!h]
% \small
% \centering
% \resizebox{0.8\textwidth}{!}
% {
% % \begin{tabular}{|p{20em}|C{3.5em}|C{4.25em}|C{10em}|} \hline
% \begin{tabular}{|l|p{18em}||c||c|c|c|c|c|c|c|}
% \hline
% & & & \multicolumn{7}{c|}{\bf \em Predicted} \\ \cline{4-10}

% & \bf Utterances & \bf Actual & $E^m$ & $E^m$ & $E^m$ & $E^m$ & $E^m$ & $E^m$ & $E^m$\\ \hline \hline

% 1 & \begin{hindi} अरे बुढ़ापे में मैं तुम्हें खुद ले के जाता।अरे बुढ़ापे में मैं तुम्हें खुद ले के जाता। \end{hindi}
% & S & f & NS & NS & NS & NS & NS & NS \\ \hline

% 2 & \beginये दिलरुबा कहता है ना कि पिछले जन्म में वो छोटूमल मोटूमल करोड़पति का एकलौता बेटा था , राइट? & S & f & NS & NS & NS & NS & NS & NS \\ \hline

% 3 & स्टाफ वालों! मेरा मतलब
% & S & f & NS & NS & NS & NS & NS & NS \\ \hline

% 4 & कुछ याद आया? कुछ याद आया?
% & S & f & NS & NS & NS & NS & NS & NS \\ \hline

% 5 & जाते वक्त ऐसी अशुभ बातें नहीं करते।
% & S & f & NS & NS & NS & NS & NS & NS \\ \hline



% \end{tabular}
% }
% % \caption{Some incorrectly predicted samples by the proposed model.}
% \caption{Error Analysis: Some incorrectly predicted samples by the proposed model}
% \label{tab-error_analysis}
% \end{table*}


==> tex/error_analysis_wrong_prediction.tex <==
\begin{table}[!h]
\small
\centering
\resizebox{0.49\textwidth}{!}
{
% \begin{tabular}{|p{20em}|C{3.5em}|C{4.25em}|C{10em}|} \hline
\begin{tabular}{|l|p{18em}||c||c|c| }
\hline
& & & \multicolumn{2}{c|}{\bf \em Predicted} \\ \cline{4-5}

& \bf  & \bf  & \bf Unimodal & \bf Multimodal \\ 
& \bf Utterances & \bf Actual & \bf (T) & \bf (T+V+A) \\ \hline \hline

1 & \begin{hindi} ये लोग मुझे बहुत मार रहे हैं। \end{hindi}
& humor & \textcolor{red}{non-humor} & \textcolor{red}{non-humor} \\ \hline

2 & \begin{hindi} हाय, टोटो! \end{hindi} 
& non-humor & non-humor & \textcolor{red}{humor} \\ \hline

3 & \begin{hindi} ये पिंकी लाई। \end{hindi} 
& humor & humor & \textcolor{red}{non-humor} \\ \hline

4 & \begin{hindi} अरे भाई, मेरी असली वाली गन यहीं छूट गई। \end{hindi} 
& non-humor & \textcolor{red}{humor} & \textcolor{red}{humor} \\ \hline

5 & \begin{hindi} कौन सी असली है कौन सी नकली है। \end{hindi} 
& non-humor & non-humor & \textcolor{red}{humor}  \\ \hline

\end{tabular}
}
% \caption{Some incorrectly predicted samples by the proposed model.}
\caption{Some incorrectly predicted samples}
\label{tab-error_analysis_wrong_prediction}
\end{table}


% \begin{table}[!h]
% \small
% \centering
% \resizebox{0.49\textwidth}{!}
% {
% % \begin{tabular}{|p{20em}|C{3.5em}|C{4.25em}|C{10em}|} \hline
% \begin{tabular}{|l|p{15em}||c||c|c|c|c|c|c|c| }
% \hline
% & & & \multicolumn{7}{c|}{\bf \em Predicted} \\ \cline{4-10}

% & \bf Utterances & \bf Actual & \bf T & \bf A & \bf V & \bf TV & \bf TA & \bf AV & \bf TAV \\ \hline \hline

% 1 & \begin{hindi} ये लोग मुझे बहुत मार रहे हैं। \end{hindi}
% & H & NH & NH & H & NH & NH & H & NH\\ \hline

% 2 & \begin{hindi} हाय, टोटो! \end{hindi} 
% & H & NH & NH & H & NH & NH & H & NH\\ \hline

% 3 & \begin{hindi} ये पिंकी लाई। \end{hindi} 
% & H & NH & NH & H & NH & NH & H & NH\\ \hline

% 4 & \begin{hindi} अरे भाई, मेरी असली वाली गन यहीं छूट गई। \end{hindi} 
% & H & NH & NH & H & NH & NH & H & NH\\ \hline

% 5 & \begin{hindi} कौन सी असली है कौन सी नकली है। \end{hindi} 
% & H & NH & NH & H & NH & NH & H & NH\\ \hline

% \end{tabular}
% }
% % \caption{Some incorrectly predicted samples by the proposed model.}
% \caption{Some incorrectly predicted samples}
% \label{tab-error_analysis_wrong_prediction}
% \end{table}


==> tex/hyperParameters.tex <==
\begin{table}[!h]
\centering
\resizebox{0.48\textwidth}{!}
{\begin{tabular}{|l|c|c|}
\hline
\bf Parameters &  \bf MISA w/ DialogueRNN & \bf MISA w/ bcLSTM \\ \hline \hline
GRU and LSTM & 900N, D=0.1 & 2$\times$900N, D=0.5 \\
Dense layer & 150N, D=0.1 & 2$\times$100N, D=0.5 \\
Activations &  \multicolumn{2}{c|}{\textit{ReLu}} \\
Optimizer & \multicolumn{2}{c|}{\textit{Adam} (\textit{lr=1e-4})} \\
Outputs & \multicolumn{2}{c|}{\textit{Softmax} (\textit{Humor})}\\
Loss & \multicolumn{2}{c|}{\textit{BCE} (\textit{Humor})}\\
Batch & \multicolumn{2}{c|}{\textit{16}} \\
Epochs & \multicolumn{2}{c|}{\textit{60}} \\ \hline
% \#Segments (k) & 50 & 25 \\ \hline 
\end{tabular}}
\caption{Model configurations}
\label{tab:param}
\end{table} 






% \begin{table}[ht!]
% \centering
% \resizebox{0.48\textwidth}{!}
% {\begin{tabular}{|l|c|c|}
% \hline
% \bf \em Parameters &  \bf \em Speaker Dependent & \bf \em Speaker Independent\\ \hline \hline
% Bi-GRU & \multicolumn{2}{c|}{2$\times$50 \textit{neurons}, \textit{dropout=0.7}} \\
% Dense layer & \multicolumn{2}{c|}{200 \textit{neurons}, \textit{dropout=0.3}} \\
% Activations &  \multicolumn{2}{c|}{\textit{ReLu}} \\
% Optimizer & \multicolumn{2}{c|}{\textit{Adam} (\textit{lr=0.001})} \\
% Output & \multicolumn{2}{c|}{\textit{Softmax} (Sent, Sar) \& \textit{Sigmoid} (Emo)} \\
% \multirow{2}{*}{Loss} & \multicolumn{2}{c|}{\textit{Categorical cross-entropy} (Sent, Sar)}\\
% &  \multicolumn{2}{c|}{\textit{Binary cross-entropy} (Emo)} \\
% Batch & \multicolumn{2}{c|}{\textit{32}} \\
% Epochs & \multicolumn{2}{c|}{\textit{200}} \\ \hline
% % \#Segments (k) & 50 & 25 \\ \hline 
% \end{tabular}}
% \caption{Model configurations}
% \label{tab:param}
% \end{table} 

==> tex/results_analysis_MISA_DRNN.tex <==
\begin{table}[!h]
\centering
\resizebox{0.25\textwidth}{!}
{    
\begin{tabular}{|c|c|c|c|}
% \begin{tabularx}{\linewidth}{|c|*{3}{X|}}
\hline

\multicolumn{4}{|c|}{\bf \em  W/ Context and W/o Speaker} \\ \hline \hline

\multicolumn{1}{|c|}{\bf \em Labels} & \bf P & \bf R & \bf F1  \\ \hline 
\bf \em T    & 67.21 & 68.31  & 67.84 \\
\bf \em A    & 57.91 & 59.10  &  58.52   \\
\bf \em V    & 55.16 &  57.32 &  56.74  \\ \hline
\bf \em T+V  & 70.03 & 70.61   &  70.31 \\
\bf \em T+A  & 69.70 &  69.90 & 69.63   \\
\bf \em A+V  & 61.70 & 63.21  &    62.44 \\ \hline
\bf \em T+V+A & \bf 71.21 & \bf 72.11  & \bf 71.67  \\


\hline
\end{tabular}
}
% \caption{Results for \textit{w/ context and w/o speaker} setup for MISA+DialogueRNN}
\caption{Results for MISA+DialogueRNN}
\label{tab:M_DRNN}
\end{table}



==> tex/results_analysis_MISA_bcLSTM.tex <==
\begin{table}[!h]
\centering
\resizebox{0.25\textwidth}{!}
{    
\begin{tabular}{|c|c|c|c|}
% \begin{tabularx}{\linewidth}{|c|*{3}{X|}}
\hline

\multicolumn{4}{|c|}{\bf \em  W/ Context and W/o Speaker} \\ \hline \hline

\multicolumn{1}{|c|}{\bf \em Labels} & \bf P & \bf R & \bf F1  \\ \hline 
\bf \em T    & 66.27 &  66.51 &  66.38   \\
\bf \em A    & 57.51 & 58.92  &  58.21   \\
\bf \em V    & 53.13 &  55.21 &  54.19   \\ \hline
\bf \em T+V  & 67.74 &  68.89 &  68.31   \\
\bf \em T+A  & 67.41 &  68.12 &  67.75   \\
\bf \em A+V  & 59.61 &  61.23 &  60.40   \\ \hline
\bf \em T+V+A & \bf  69.04 & \bf  69.83& \bf 69.43  \\


\hline
\end{tabular}
}
\caption{Results for MISA+bcLSTM}
\label{tab:M_bcLSTM}
\end{table}



==> tex/results_analysis_wC_wS.tex <==
\begin{table}[!h]
\centering
\resizebox{0.25\textwidth}{!}
{    
\begin{tabular}{|c|c|c|c|}
% \begin{tabularx}{\linewidth}{|c|*{3}{X|}}
\hline

\multicolumn{4}{|c|}{\bf \em  W/ Context and W/ Speaker} \\ \hline \hline

\multicolumn{1}{|c|}{\bf \em Labels} & \bf P & \bf R & \bf F1  \\ \hline 
\bf \em T    & 69.9 &  69.7 &  69.6   \\
\bf \em A    & 69.1 &  68.0 &  67.4   \\
\bf \em V    & 75.1 &  74.2 &  74.0   \\ \hline
\bf \em T+V  & 75.1 &  74.8 &  74.7   \\
\bf \em T+A  & 70.6 &  70.3 &  70.1   \\
\bf \em A+V  & 76.1 &  75.7 &  75.6   \\ \hline
\bf \em T+V+A & \bf 77.9 & \bf 76.9 & \bf 76.7  \\


\hline
\end{tabular}
}
\caption{Results for \textit{w/ context and w/ speaker} setup}
\label{tab:wC_wS}
\end{table}



==> tex/results_analysis_woC_wS.tex <==
\begin{table}[!h]
\centering
\resizebox{0.25\textwidth}{!}
{    
\begin{tabular}{|c|c|c|c|}
% \begin{tabularx}{\linewidth}{|c|*{3}{X|}}
\hline

\multicolumn{4}{|c|}{\bf \em  W/o Context and W/ Speaker} \\ \hline \hline

\multicolumn{1}{|c|}{\bf \em Labels} & \bf P & \bf R & \bf F1  \\ \hline 
\bf \em T    & 69.9 &  69.7 &  69.6   \\
\bf \em A    & 69.1 &  68.0 &  67.4   \\
\bf \em V    & 75.1 &  74.2 &  74.0   \\ \hline
\bf \em T+V  & 75.1 &  74.8 &  74.7   \\
\bf \em T+A  & 70.6 &  70.3 &  70.1   \\
\bf \em A+V  & 76.1 &  75.7 &  75.6   \\ \hline
\bf \em T+V+A & \bf 77.9 & \bf 76.9 & \bf 76.7  \\


\hline
\end{tabular}
}
\caption{Results for \textit{w/o context and w/ speaker} setup}
\label{tab:woC_wS}
\end{table}



==> tex/results_analysis_woC_woS.tex <==
\begin{table}[!h]
\centering
\resizebox{0.25\textwidth}{!}
{    
\begin{tabular}{|c|c|c|c|}
% \begin{tabularx}{\linewidth}{|c|*{3}{X|}}
\hline

\multicolumn{4}{|c|}{\bf \em  W/o Context and W/o Speaker} \\ \hline \hline

\multicolumn{1}{|c|}{\bf \em Labels} & \bf P & \bf R & \bf F1  \\ \hline 
\bf \em T    & 69.9 &  69.7 &  69.6   \\
\bf \em A    & 69.1 &  68.0 &  67.4   \\
\bf \em V    & 75.1 &  74.2 &  74.0   \\ \hline
\bf \em T+V  & 75.1 &  74.8 &  74.7   \\
\bf \em T+A  & 70.6 &  70.3 &  70.1   \\
\bf \em A+V  & 76.1 &  75.7 &  75.6   \\ \hline
\bf \em T+V+A & \bf 77.9 & \bf 76.9 & \bf 76.7  \\


\hline
\end{tabular}
}
\caption{Results for \textit{w/o context and w/o speaker} setup}
\label{tab:woC_woS}
\end{table}


